Photometric Stability of an EMCCD Camera at 1-s Exposures

We present the results of testing an iXonUltra 888 EMCCDcamera to determine the operating parameters for short-exposure photometry of stars. As a result of the testing, those camera modes were selected in which the temporal instability of the electron multiplication charge does not significantly affect the light curves. In addition, the photometry of the eclipsing variable star ZTFJ 0038+2030, obtained with the Zeiss-1000 telescope of the Special Astrophysical Observatory of the Russian Academy of Sciences, is presented. We have shown the advantages and disadvantages of 1-s exposures for studying variable stars.

==> engnames.tex <==
%
% engnames.tex 11.11.2005
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{ACKNOWLEDGMENTS}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{PACS~numbers:~}%
\def\@ydk@name{~}%
\def\@keywords@name{Key~words:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{revised }%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
\makeatother
\endinput

